Simple and Effective Transfer Learning for Neuro-Symbolic Integration

Deep Learning (DL) techniques have achieved remarkable successes in recent years. However, their ability to generalize and execute reasoning tasks remains a challenge. A potential solution to this issue is Neuro-Symbolic Integration (NeSy), where neural approaches are combined with symbolic reasoning. Most of these methods exploit a neural network to map perceptions to symbols and a logical reasoner to predict the output of the downstream task. These methods exhibit superior generalization capacity compared to fully neural architectures. However, they suffer from several issues, including slow convergence, learning difficulties with complex perception tasks, and convergence to local minima. This paper proposes a simple yet effective method to ameliorate these problems. The key idea involves pretraining a neural model on the downstream task. Then, a NeSy model is trained on the same task via transfer learning, where the weights of the perceptual part are injected from the pretrained network. The key observation of our work is that the neural network fails to generalize only at the level of the symbolic part while being perfectly capable of learning the mapping from perceptions to symbols. We have tested our training strategy on various SOTA NeSy methods and datasets, demonstrating consistent improvements in the aforementioned problems.

==> chapters/background.tex <==
NeSy systems\footnote{\sm{ this seems wrong to me}: \ad{it is correct, but maybe it is convenient to say this at the level of related works} Here we refer to NeSy systems in the specific context where the symbolic reasoner is employed to infer new facts from the given knowledge. This excludes methods like LTN where the knowledge is merely used to constrain the outputs of the neural network. It should be noted that not all NeSy systems operate in this manner.} can be seen as composition of \emph{perception functions} with a \emph{symbolic function}. A perception function $f: \mathcal{X} \rightarrow \Sym$ takes in raw unstructured data $x \in \mathcal{X}$ as input (e.g. images, natural language text etc.) and maps it to symbols $\Sym$ of a formal language. A symbolic function $g:\Sym^{n} \rightarrow \Sym$, representing a symbolic reasoner with expert knowledge,
% or a set of constraints
takes $n$ symbols as input and gives out a new symbol. Most NeSy systems can be represented as a composition of the perception and symbolic function, of the form $g(f_1(x_1),\dots f_n(x_n))$, where $x_i$ are the perception inputs and $f_i$ are the perception functions mapping $x_i$ to a symbol in $\Sym$. In most NeSy systems $f_i$ is a NN with learnable parameters, whereas $g$ represents expert provided rules \cite{manhaeve2018deepproblog,winters2022deepstochlog, ILR,Daniele2019KnowledgeEN}. Recent works have also expanded towards learning both the perceptions and the symbolic function \cite{DSL,Evans}.\ad{no, Evans impara solo g, ma non f (che e' data). Bisogna aggiungere il lavoro nuovo visto a NeSy di Marra, dove anche loro imparano tutto assieme }

% The symbolic reasoner module is instead defined by its role in interpreting and implementing the symbolic knowledge of the system. Depending on the method used, this may vary greatly. For example, in DPL, the reasoning module employs ProbLog, a probabilistic logic programming language, to carry out its tasks. Meanwhile, in ILR, the reasoning module utilizes propositional logic rules to perform its symbolic reasoning. In the case of DSL, the traditional reasoner is replaced with a symbolic function. This $n$-ary symbolic function $g: \Sym^{n} \rightarrow \Sym$ serves the role of the reasoner. It maps an input of $n$ symbols to other symbols, thereby effectively reasoning over the input symbols. This approach, like others in the realm of NeSy systems, showcases the diversity and adaptability of these systems in handling unstructured data and symbolic reasoning.

In this paper, we focus  on NeSy systems, where logical reasoning takes place under fuzzy logic semantics. Fuzzy logic relaxes the notion boolean truth values to fuzzy truth values in $[0,1]$. The semantics of logical connectives (i.e. $\land, \lor, \neg$ e.t.c.) under different fuzzy logic semantics correspond to different types of aggregation functions over fuzzy truth values. In this paper, we focus on two fuzzy logic-based NeSy systems, namely \emph{Deep Symbolic Learning} (DSL)~\cite{DSL} and \emph{Iterative Local Refinement} (ILR)~\cite{ILR}.



% \sm{NeSy systems can be seen as composition of \emph{perception functions}  and \emph{symbolic functions}, in varying orders of complexity. A perception function $f$ takes in raw unstructured data $x \in \mathcal{X}$ as input (e.g. images, natural language text e.t.c) and maps it to symbols $\Sym$ of the logical language of the NeSy system. An $n$-ary symbolic function $g: \Sym^{n} \rightarrow \Sym$ on the other hand maps an input of $n$ symbols to other symbols, by reasoning over the input symbols. Symbolic functions in NeSy systems represent logical reasoning. In this paper our focus is on NeSy systems, where the logical reasoning takes place under fuzzy logic semantics. Fuzzy logic relaxes the notion boolean truth values to fuzzy truth values in $[0,1]$. The semantics of logical connectives (i.e. $\land, \lor, \neg$ e.t.c.) under different fuzzy logic semantics correspond to different types of aggregation functions over fuzzy truth values. In this paper we focus on two prominent fuzzy logic based NeSy systems namely \emph{Deep Symbolic Learning}(DSL) \cite{DSL} and \emph{Iterative Local Refinement}(ILR) \cite{ILR}. }

\paragraph{Iterative Local Refinement.}
Iterative Local Refinement (ILR) is an algorithm that iteratively optimizes a given propositional logic formula $\phi$ starting from a vector $\bf t$ that represents an initial interpretation of the propositional variables in $\phi$~\cite{ILR}. ILR is very similar to the Back-Propagation (BP) algorithm, where the backward pass employs \emph{refinement functions} instead of gradients. A refinement function is defined as the solution of the following optimization problem:
$
    % \label{eq:optim-problem}
    % \begin{aligned}
        % \textrm{For all } \quad & {\bf t}\in [0,1]^n, \revis{\varphi} \in [0, 1]  \\
        \min_{\boostv} \ \|\boostv - \truth\| \ \ 
        \textrm{s.t.} \  \op_\varphi(\boostv) = \revis{\varphi}
        % ,  \\
        % & 0 \leq  \boosts_i \leq 1
        % & \boosts_i=\truths_i, i\in F 
    % \end{aligned}
$,
where $\varphi$ is a fuzzy operator, $\revis{\varphi}$ is the target value, i.e., the operator truth value after the optimization; and $\op_\varphi$ is the function that provides the interpretation (truth value) for $\varphi$ for the vector $\boostv$. 

% Intuitively, given an operator $\varphi$, an initial interpretation of the  and a target value $\revis{\varphi}$, the refinement function calculates

ILR provides results similar to BP when optimizing the knowledge. However, the required amount of optimization steps (i.e., iterations) are much smaller (typically no more than 4 steps). If the logical operators are defined by differentiable functions, then ILR steps are also differentiable. Hence, ILR provides a general method for adding fuzzy logic constraints into NN frameworks. Each step in ILR can be inserted in the NN architecture as an additional layer, allowing optimizing the knowledge within a neural model.

% Similarly to LTN, in ILR the knowledge represents constraints on the output of the NN. However, differently from LTN, ILR can be employed in the same contexts as DeepProblog. Indeed, it has been shown that the refinement function for the residuum (implication in fuzzy logic) behaves similarly to \emph{modus ponens}, allowing to adopt ILR to perform inference~\cite{ILR}. Note that, while ILR is defined for multiple semantics, only for the G\"{o}del one the residuum is implemented. Hence, our experiments make use only of the G\"{o}del semantics, where the conjunction is represented with the min operator and the disjunction as the max.
% % $\mathcal{I}(A \land B) = \top(\mathcal{A},\mathcal{B}) = min(\mathcal{I}(A),\mathcal{I}(B))$, where $\mathcal{I}$ represents the interpretation of a formula. 
% % Similarly, the disjunction is represented with the max operator. 
% Finally, the implication is interpreted using the G\"{o}del Residuum.
% For more details on G\"{o}del semantics and fuzzy logic in general, see~\cite{klement2000mcsiar}.

%\setlength{\intextsep}{1pt}%
%\setlength{\columnsep}{1pt}%


\paragraph{Deep Symbolic Learning.}
DSL takes inspiration from the concept of policy functions in reinforcement learning (RL), specifically from the greedy policy approach~\cite{DSL}. However, it's crucial to note that DSL operates in a different context, applying these principles within NeSy rather than RL. In a traditional greedy policy, the most promising option is selected to guide the learning trajectory. DSL adopts this core principle but adjusts the selection space from actions, as typically found in RL, to internal model symbols in NeSy. In this altered context, the output of the neural network in DSL isn't treated as an expected reward, as would be the case in RL. Instead, it's interpreted as a fuzzy truth value, embodying the degree of truth rather than a binary distinction.

% A unique feature of DSL is its capacity to handle simultaneous multiple discrete choices within the model. 
In DSL each chosen symbol, assigned a fuzzy truth value, represents a decision made by the policy. This concept diverges from conventional greedy policies, where a single best option is selected, enabling an ensemble of symbol choices within the model instead. These fuzzy truth values are then aggregated using principles of fuzzy logic. This aggregated score indicates the \say{truthfulness} of the collective set of decisions, offering a holistic representation of the model's state.

Finally, DSL also allows for learning the symbolic rules themselves. This is done by selecting the rules that maximize the truth value of the symbolic mappings. Note that learning simultaneously both perception functions and symbolic rules poses additional challenges. For this reason, DSL is strongly limited by convergence issue with complex perceptions and knowledge.


 % The key idea  behind DSL is to adapt reinforcement learning policies to the NeSy context: given the NN predictions $\bf t$ over a set of symbols such that $\sum_i t_i = 1$, DSL uses the greedy policy $\pi({\bf t}) = argmax_i t_i$ 
% (during training we use epsilon-greedy policy to enforce a better exploration) 
% to select a single discrete symbol, and the function $\mu({\bf t}) = max_i t_i$ to select the corresponding value in $\bf t$, interpreted as a truth value of the chosen symbol under a fuzzy logic semantics. For evaluating truth value of a given symbolic rule, given as expert-knowledge, these truth values are aggregated w.r.t  fuzzy logic semantics. 


% Fuzzy Logic is a multi-valued generalization of classical logic, where truth values are reals in the range $[0,1]$. In this work, we will only be dealing with conjunctions, which in fuzzy logic are interpreted using \emph{t-norms}. A t-norm $t:[0,1]\times[0,1]\rightarrow [0,1]$ is a function that,  given the truth values $t_1$ and $t_2$ for two logical variables, computes the truth value of their conjunction. In this paper, we will exploit \godel\ t-norm, which defines the truth value of a conjunction as the minimum of $t_1$ and $t_2$.


% \paragraph{Notation.}We denote sets with math calligraphic font and its elements with corresponding indexed lower case letter, e.g., $\Sym = \{ s_i | \forall i \in \mathbb{N}, 0 < i \leq k \}$, where $k = |\Sym|$ is the cardinality of the set. 
% Tensors are denoted with capital bold letters (e.g. $\G$) and the $[ \dots ]$ operator is used to index values in a tensor. For instance, given a matrix $\G \in \mathbb{R}^{10 \times 10}$, the element $\G[1, 2]$ corresponds to the entry in row 1 and column 2 of $\G$. Similar to python syntax, we introduce the colon symbol for indexing slices of a tensor. As an example, $\G[1, \ :]$ corresponds to the vector $\langle \G[1, 1], \dots, \G[1, 10] \rangle$. We use a bar on top of functions and elements of a set to denote a tuple of functions and elements, respectively. For instance, $\bar{s} = \bar{f}(\bar{x})$ is equivalent to:
% $$(s_1, \dots, s_n) = (f_1(x_1), \dots, f_n(x_n))$$
% Note that the length $n$ of the tuple is omitted from the bar notation since it will always be clear from the context.  

%\paragraph{Fuzzy Logic.}









% Perception functions in NeSy systems are represented by Neural Networks, whereas different proposals for modelling the symbolic function have been proposed \cite{ProbLog, LTN, T_norm_Driven_loss_functuions, tsamoura2021neural, SAT_Net_Solve}. 

% These proposals can be largely classified into probabilistic logic based NeSy systems (P-NeSy) and Fuzzy logic based NeSy systems


% A key challenge to learning in NeSy systems is that they deal with both discrete and continuous data attributes. Furthermore, 





% They offer a promising direction for addressing complex problems by leveraging the robustness of symbolic methods with the adaptability of neural networks. However, despite the potential of NeSy systems, there are several challenges that need to be addressed before they can be effectively deployed in a wide range of applications.

% One of the primary concerns in NeSy systems is scalability\sm{citations}. Probabilistic logic-based (P-NeSy) \sm{citations} methods often struggle to scale to large problem domains due to their computational complexity. On the other hand, fuzzy logic-based methods\sm{citations}  offer better efficiency, but they are prone to reasoning shortcuts \ad{and local minima}. This issue is particularly pronounced in fuzzy logic-based NeSy methods (F-NeSy), \ad{raising questions about their reliability.}

% \ad{Another challenge faced by NeSy systems is the lack of convergence when dealing with complex knowledge, especially when learning simoultaneously perception function and symbolic knowledge, e.g., in Deep Symbolic Learning (DSL).} This issue poses a significant barrier to the widespread adoption of F-NeSy methods, as it limits their applicability to complex and real-world problems.

% In this paper, we propose a novel strategy to overcome these challenges by introducing an Auxiliary Model (AM) to F-NeSy methods. The AM is a standard neural network that is designed to address the scalability and convergence issues inherent in current NeSy approaches. Our strategy involves training the AM using the same supervision as the NeSy Model, focusing on the downstream task. \ad{This approach is highly generalizable, applicable to a wide range of NeSy systems and problem domains.}

% \ad{aggiungere intro ILR e DSL}

% The AM and the NeSy Model share common parameters, specifically the perceptual function. This shared architecture enables the two models to \ad{synergistically learn and adapt from each other.} In essence, the AM quickly learns the perceptual aspect of the problem but fails to generalize in the symbolic part. On the other hand, DSL and ILR methods exhibit generalization and speed, but they often fall into local minima (ILR) or fail to converge (DSL).

% By learning both models together, we effectively transfer the knowledge about perceptions from the AM to the ILR (or DSL) method. This results in a system that combines the best of both worlds: the fast perceptual learning of the AM with the robust symbolic reasoning capabilities of ILR and DSL methods. Our approach offers a promising direction for addressing the \ad{scalability and} convergence challenges faced by F-NeSy systems, paving the way for their broader application in tackling complex problems.

% \sm{Summing up, in this paper...}


% \subsection{Logic Tensor Networks}
% Logic Tensor Networks \cite{LTN} provide a computational framework for Neuro-Symbolic integration based in \emph{Real Logic}: a variant of fuzzy-logic, where domains are interpreted as tensors in a real field. This means that every object denoted by a constant, variable, and term, is interpreted as a real-valued tensor. Functions in real logic are simply represented as functions over real valued tensors, and predicates are represented as mappings from tensors to values in the interval $[0,1]$. Given a formula in Real logic, it's truth value under different instantiation of the domain are evaluated using  fuzzy-logic semantics. 



% Real Logic provides a skeleton for specifying logical formulas in terms of real-valued functions. The  semantics of t


% \ad{rimuovere gli esempi. Introdurre direttamente sulla parte sperimentale}
% \begin{example}[Sum task]
% \label{ex: MNIST_SUM}
% Let $\Sym_1$ and $\Sym$ be the following set of symbols: 
%   $\Sym_1$ are the integers from $0$ to $9$ and $\Sym$ is the set of integers from $0$ to
%   $18$. Let us have a training set, consisting of tuples $(x_1,
%   x_2 ,y)$ where $x_1$ and $x_2$ are images of handwritten
%   digits  and
%   $y$ is the result of adding the digits $x_1$ and $x_2$. Our goal is to learn the Direct NeSy-function:
%   $$
%   \phi(x_1, x_2) = g(f(x_1),f(x_2))
%   $$
%   where $f$ is handwritten digit classifiers. Hence, our goal is to learn $f$ and $g$ with supervision provided only on $g(\bar{f}(\bar{x}))$.
% \end{example}

% \begin{example}[Multi-digit Sum]
% \label{ex:multi_digit}
% Let $\Sym$ be the set of symbols corresponding to the integers from 0 to 9, and $\Sym_c = \{s_0, s_1\}$ another set of symbols. We have a training set composed of pairs of multi-digit numbers and their sum as labels. Each number is represented by a list of MNIST digit images. The goal is to learn the NeSy function $\phi$ that computes the sum of the given numbers. Similarly to Example~\ref{ex: parity}, the NeSy function can be defined recursively. However, in this case, there are two symbolic functions, which compute the single-digit summation modulo 10 and the carry, respectively. For more details, we refer the reader to the Supplementary Material.
% \end{example}
